Speeding up Routing Schedules on Aisle-Graphs with Single Access

In this paper, we study the Orienteering Aisle-graphs Single-access Problem (OASP), a variant of the orienteering problem for a robot moving in a so-called single-access aisle-graph, i.e., a graph consisting of a set of rows that can be accessed from one side only. Aisle-graphs model, among others, vineyards or warehouses. Each aisle-graph vertex is associated with a reward that a robot obtains when visits the vertex itself. As the robot's energy is limited, only a subset of vertices can be visited with a fully charged battery. The objective is to maximize the total reward collected by the robot with a battery charge. We first propose an optimal algorithm that solves OASP in O(m^2 n^2) time for aisle-graphs with a single access consisting of m rows, each with n vertices. With the goal of designing faster solutions, we propose four greedy sub-optimal algorithms that run in at most O(mn (m+n)) time. For two of them, we guarantee an approximation ratio of 1/2(1-1/e), where e is the base of the natural logarithm, on the total reward by exploiting the well-known submodularity property. Experimentally, we show that these algorithms collect more than 80% of the optimal reward.

==> T-RO 2020 - RevisedVersion/macro.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}

\newcommand{\descr}[1]{\medskip\noindent\textbf{#1}.}
\renewcommand{\paragraph}{\descr}

\newcommand{\todo}[1]{\textcolor{blue}{\ding{46}{\sf}~\textbf{#1}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

% \newcommand{\aislegraph}{A\xspace}

\newcommand{\call}[1]{\mathcal{#1}}

\newcommand{\cristina}[1]{{\color{red}{-CP: #1-}}}
\newcommand{\francesco}[1]{{\color{blue}{-FBS: #1-}}}
\newcommand{\FC}[1]{{\color{green}{-FC: #1-}}}
\newcommand{\alfredo}[1]{{\color{purple}{-AN: #1-}}}
\newcommand{\SC}[1]{{\color{teal}{-SC: #1-}}}
\newcommand{\revision}[1]{{\color{black}{#1}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\imax}{\ensuremath{i\textsubscript{max}}\xspace}
\newcommand{\rmax}{\ensuremath{r\textsubscript{max}}\xspace}
\newcommand{\mmin}{\ensuremath{m\textsubscript{min}}\xspace}
\newcommand{\vcycle}{\ensuremath{V\textsubscript{cycle}}\xspace}
\newcommand{\val}{\ensuremath{val}\xspace}
\newcommand{\dist}{\ensuremath{dist}\xspace}
\newcommand{\best}{\ensuremath{best}\xspace}
\newcommand{\bres}{\ensuremath{B\textsubscript{res}}\xspace}

\newcommand{\ofri}{\textsc{OFr-I}\xspace}
\newcommand{\gfr}{\textsc{GFr}\xspace}
\newcommand{\gpr}{\textsc{GPr}\xspace}
\newcommand{\hgc}{\textsc{HGc}\xspace}

\newcommand{\ofrilong}{{Optimal Full-Row Improved}\xspace}
\newcommand{\gfrlong}{{Greedy Full-Row}\xspace}
\newcommand{\gprlong}{{Greedy Partial-Row}\xspace}
\newcommand{\hgclong}{{Heuristic General-case}\xspace}

\newcommand{\optsc}{\textsc{OptSa}\xspace} % Optimum Single Access
\newcommand{\gdyme}{\textsc{GdyME}\xspace} % Greedy Max Element
\newcommand{\gdymc}{\textsc{GdyMC}\xspace} % Greedy Max Cumulative
\newcommand{\apxmre}{\textsc{ApxMRE}\xspace} % Approximate Max Ratio Element
\newcommand{\apxmrc}{\textsc{ApxMRC}\xspace} % Approximate Max Ratio Cumulative

\newcommand{\optsclong}{{Optimum Single Access}\xspace}
\newcommand{\gdymelong}{{Greedy Max Element}\xspace}
\newcommand{\gdymclong}{{Greedy Max Cumulative}\xspace}
\newcommand{\apxmrelong}{{Approximate Max Ratio Element}\xspace}
\newcommand{\apxmrclong}{{Approximate Max Ratio Cumulative}\xspace}

\newcommand{\prob}{OASP\xspace} % Orienteering Aisle-graphs Single-access Problem
\newcommand{\problong}{Orienteering Aisle-graphs Single-access Problem\xspace}

\newcommand{\sol}{\textsc{SOL}\xspace}
\newcommand{\opt}{\textsc{OPT}\xspace}
\newcommand{\alg}{\textsc{ALG}\xspace}

